A Rapidly Deployable Classification System using Visual Data for the Application of Precision Weed Management

In this work we demonstrate a rapidly deployable weed classification system that uses visual data to enable autonomous precision weeding without making prior assumptions about which weed species are present in a given field. Previous work in this area relies on having prior knowledge of the weed species present in the field. This assumption cannot always hold true for every field, and thus limits the use of weed classification systems based on this assumption. In this work, we obviate this assumption and introduce a rapidly deployable approach able to operate on any field without any weed species assumptions prior to deployment. We present a three stage pipeline for the implementation of our weed classification system consisting of initial field surveillance, offline processing and selective labelling, and automated precision weeding. The key characteristic of our approach is the combination of plant clustering and selective labelling which is what enables our system to operate without prior weed species knowledge. Testing using field data we are able to label 12.3 times fewer images than traditional full labelling whilst reducing classification accuracy by only 14%.

==> body/results/results.tex <==
%\section{Results}\label{sec:results}
%\begin{figure}[t]
%	\centering
%	\setlength{\fboxsep}{0pt}
	
%	\begin{subfigure}[b]{0.45\linewidth}
%		\centering
%		\fbox{\includegraphics[width=\linewidth]{results/labelling_plot_redlands.jpg}}
%		\caption{Redlands Labelling Results}
%	\end{subfigure}
%	\begin{subfigure}[b]{0.45\linewidth}
%		\centering
%		\fbox{\includegraphics[width=\linewidth]{results/labelling_plot_flavia.jpg}}
%		\caption{Flavia Labelling Results}
%	\end{subfigure}
%	\caption{Overall labelling accuracy vs number of exemplars labelled plots for the Redlands (a) and Flavia (b) datasets. Best viewed in colour.}
%	\label{fig:results:label}
%\end{figure}

%\begin{figure}[t]
%	\centering
%	\setlength{\fboxsep}{0pt}
%	
%	\begin{subfigure}[b]{0.45\linewidth}
%		\centering
%		\fbox{\includegraphics[width=\linewidth]{results/classification_plot_redlands.jpg}}
%		\caption{Redlands Classification Results}
%	\end{subfigure}
%	\begin{subfigure}[b]{0.45\linewidth}
%		\centering
%		\fbox{\includegraphics[width=\linewidth]{results/classification_plot_flavia.jpg}}
%		\caption{Flavia Classification Results}
%	\end{subfigure}
%	\caption{Overall classification accuracy vs number of exemplars labelled plots for the Redlands (a) and Flavia (b) datasets. Best viewed in colour.}
%	\label{fig:results:class}
%\end{figure}

%In our work we evaluate the labelling techniques described in Section~\ref{sec:method:label:test_setup} in terms of labelling accuracy and classification accuracy across both the Redlands and Flavia datasets.
%As our focus is on trying to label and classify plants with as little human interaction as possible, we summarise labelling and classification accuracy versus the number of exemplars labelled by humans in Figures~\ref{fig:results:label}~and~\ref{fig:results:class} respectively.
%As \KM, \LP, and \LLP~all require a predefined number of clusters/exemplars, we present a range of different numbers of exemplars for these methods here.
%The number of exemplars increases in intervals of 10\% of the total number of training images.
%This range of values demonstrates the rate at which labelling accuracy is increases as an effect of labelling more images.
%For \LP~and \LLP we also demonstrate a scenario where the number of exemplars is equal to the number of exemplars attained through \AP~and \APR.
%This is to allow a more direct comparison between a randomised set of exemplars and a more structured choice of exemplar.
%As the fine-tuning process that we use for training our classifier can be quite time-intensive, we only demonstrate the two lowest levels of labelling (10\% and 20\% of the number of samples) as well as the scenarios where the number of exemplars is equal to that of \AP~and \APR.
%We also demonstrate classification accuracy for \Full~to show the maximum classification accuracy that we could expect when trained on the given training set.
%Analysing the results presented in Figures~\ref{fig:results:label}~and~\ref{fig:results:class}, we can make several observations regarding the different methods presented for labelling and classifying data.
%\TODO{Update the legend to match the headings given in previous section}


